VideoMaMa: Mask-Guided Video Matting via Generative Prior

Generalizing video matting models to real-world videos remains a significant challenge due to the scarcity of labeled data. To address this, we present Video Mask-to-Matte Model (VideoMaMa) that converts coarse segmentation masks into pixel accurate alpha mattes, by leveraging pretrained video diffusion models. VideoMaMa demonstrates strong zero-shot generalization to real-world footage, even though it is trained solely on synthetic data. Building on this capability, we develop a scalable pseudo-labeling pipeline for large-scale video matting and construct the Matting Anything in Video (MA-V) dataset, which offers high-quality matting annotations for more than 50K real-world videos spanning diverse scenes and motions. To validate the effectiveness of this dataset, we fine-tune the SAM2 model on MA-V to obtain SAM2-Matte, which outperforms the same model trained on existing matting datasets in terms of robustness on in-the-wild videos. These findings emphasize the importance of large-scale pseudo-labeled video matting and showcase how generative priors and accessible segmentation cues can drive scalable progress in video matting research.

==> figures/3_semantic_knowledge.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{figures/source/dino_motivation.pdf}
    \vspace{-20pt}
    \caption{Sematic knowledge supplement figure placeholder.}
    \label{fig:my_label}
\end{figure}

==> figures/4_MAM_qual.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/source/main_qual.pdf}
    \vspace{-15pt}
    \caption{mam qual. (Placeholder)}
    \label{fig:mam}
\end{figure*}

==> figures/5_Conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

==> sec_11-11/5_MainResults_long.tex <==
\section{Experiments} 
\label{sec:exp}
\input{figures/4_VideoMaMa_qual}
\input{tables_11-11/mask_to_matte_main_table}

\subsection{Experimental Details}
\SO{we can move these details to supp. if we need more space.}
\paragraph{Implementation details.}
We train VideoMaMa based on the Stable Video Diffusion~\cite{svd} (SVD) model using diverse image and video matting datasets. Our two-stage training strategy employs different resolutions optimized for each stage's objective. In stage 1, we train the spatial layers of SVD on single images at high resolution (1024×1024) to capture fine-grained matting details such as hair strands and intricate boundary structures. We freeze the temporal layers during this stage to focus learning on spatial precision. In stage 2, we freeze the learned spatial layers and train only the temporal layers on video sequences. To balance computational efficiency with temporal modeling, we use 3-frame clips at 704×704 resolution, which enables the model to learn temporal consistency and motion-aware matting characteristics. To inject semantic knowledge, we incorporate features from a frozen DINOv3~\cite{dinov3} encoder, aligning the DINO features with the first upsampling block of the SVD decoder. This integration provides the diffusion model with semantic understanding of object structures while preserving its generative capabilities.

\paragraph{Training details.}
For both stages, we use a batch size of 64 and a learning rate of $5 \times 10^{-5}$ with the AdamW optimizer. The training objective, $\mathcal{L}_{\text{mat}}$, combines L1 loss for pixel-wise accuracy and Laplacian loss for preserving edge sharpness and boundary details. Each stage is trained for 10,000 iterations until convergence. All experiments are conducted on NVIDIA A100 GPUs with mixed-precision training for efficiency.
SAM2-Matte is trained on the combination of existing video matting datasets and \mbox{MA-V}. Details of the existing datasets are provided in the appendix.

\subsection{Mask-Guided Video Matting}

\paragraph{Evaluation protocol.}
Following the protocol of mask-guided video matting evaluation~\cite{maggie}, we evaluate VideoMaMa on standard benchmarks to assess its generation quality and practical applicability. Since VideoMaMa requires a rough mask track to indicate the foreground object, we obtain mask tracks through various methods to simulate real-world usage scenarios. 

We evaluate two categories of input masks: (1) Synthetically Degraded Masks, where we artificially degrade ground-truth masks through downsampling (8$\times$, 32$\times$) and polygonization with varying difficulty levels (easy, hard). These degradations remove precise boundary information, mimicking imperfect user annotations or coarse segmentation outputs. (2) Model-Generated Masks from state-of-the-art video object segmentation methods such as SAM2~\cite{sam2}, representing fully automatic mask generation pipelines. This diverse set of input conditions allows us to evaluate VideoMaMa's robustness across different mask quality levels and generation methods.

We compare VideoMaMa against mask-guided matting baselines including MaGGIe~\cite{maggie}, a video mask-guided matting model, and MGM~\cite{mgmatting}, an image mask-guided matting model applied frame-by-frame. To quantify the refinement capability, we report metrics comparing both the input mask and each model's generated result against the ground-truth alpha matte, clearly demonstrating the improvement margin achieved by each method. All evaluations are conducted on video sequences with a maximum of 12 frames.

We adopt standard evaluation metrics widely used in the video matting community, including Mean Absolute Difference (MAD) for overall accuracy and Gradient error~\cite{rhemann2009perceptually} for assessing boundary quality. Results are reported on V-HIM60 Hard~\cite{maggie}, which contains complex multi-instance scenarios, and YouTubeMatte 1920$\times$1080~\cite{matanyone}, which provides high-resolution evaluation.

\paragraph{Quantitative and qualitative results.}
As shown in Table~\ref{tab:refinement_benchmark_wide}, VideoMaMa consistently outperforms existing mask-guided matting models across both synthetically degraded and model-generated masks. Our evaluation across different mask styles demonstrates that VideoMaMa can handle various types of mask inputs and produce high-quality video mattes consistently. Despite being trained exclusively on synthetic datasets, VideoMaMa shows strong generalization to diverse real-world scenarios. As shown in the qualitative results in Figure~\ref{fig:videomama_qual}, VideoMaMa not only performs well on human matting but also generalizes to a wide range of object categories and video content in in-the-wild video.

\subsection{First-Frame Mask-Guided Video Matting}
\input{tables_11-11/first_mgm_quan}
To validate the effectiveness of our large-scale pseudo video matting annotations, we evaluate SAM2-Matte as a representative model to assess \mbox{MA-V}'s quality. We train SAM2-Matte on a combination of existing video matting datasets and \mbox{MA-V} (see appendix for the complete dataset list). 

% \jl{remove this paragraph?} For evaluating VideoMaMa, we account for the architectural differences between methods: while MatAnyone and SAM2-Matte propagate matting results frame-by-frame with temporal context from previous frames, VideoMaMa processes a fixed number of frames simultaneously. To ensure fair comparison, we chunk the entire video into 12-frame segments with their corresponding masks, perform inference on each segment independently, and merge the results to obtain the complete video matting.

\paragraph{Evaluation protocol.}
We evaluate VideoMaMa and SAM2-Matte in a setting where a binary mask guidance is provided only for the first frame, following~\cite{matanyone}.
For VideoMaMa, the binary mask guidance across all frames is generated by propagating the mask from the first frame using SAM2~\cite{sam2}.
We employ multiple evaluation metrics: MAD for overall semantic accuracy, MSE for pixel-level error, MAD-T (trimap-based MAD) which computes MAD only within the uncertain trimap region derived from the ground-truth alpha map, and Gradient error~\cite{rhemann2009perceptually} for assessing boundary detail extraction quality. The trimap-based evaluation is particularly important as it focuses on the challenging boundary regions where precise matting is most critical. We also report the score of the binary masks produced by SAM2 to provide a baseline for the improvements achieved by VideoMaMa.

\paragraph{Quantitative and qualitative results.}
As shown in Table~\ref{tab:first_mgm_quan}, SAM2-Matte trained on the combined dataset surpasses previous state-of-the-art methods, MatAnyone~\cite{matanyone}, on challenging benchmarks: V-HIM60 Hard~\cite{maggie} and YouTubeMatte~\cite{matanyone}. This demonstrates that \mbox{MA-V} provides high-quality training data for video matting models, enabling to extract matting quality and temporal consistency over the video frames. Note that, for VideoMaMa in this experiment, we processed each of the 12-frame segments and merged the results to obtain the complete video matting.

To further evaluate the model's performance on real-world videos, we provide qualitative comparisons in Figure~\ref{fig:sam2-matte_qual}, comparing SAM2-Matte against MatAnyone. Training with \mbox{MA-V} enables the model to generate fine-grained matting results with accurate boundary details, handle objects of diverse scales and categories, and maintain strong temporal consistency across frames. These results validate that \mbox{MA-V}'s large-scale, diverse annotations effectively improve video matting quality beyond what existing datasets can achieve.

\subsection{Ablation Studies}

\paragraph{Number of inference frames.}
\input{tables/ablations/num_frames}
We evaluate VideoMaMa's performance across varying numbers of video frames to assess its generalization capability beyond the training configuration. Although VideoMaMa is trained on maximum 3 frames during training, it successfully handles diverse frame counts ranging from single frames to 24 frames at inference time. As shown in Table~\ref{tab:num_frames}, the model maintains consistent performance across different frame counts, demonstrating remarkable temporal generalization. This flexibility is particularly valuable for practical applications where video lengths vary significantly. The results indicate that our model learns robust temporal priors that transfer effectively to both shorter and longer sequences than those seen during training. 
% Furthermore, we observe that the model generalizes well to multiple resolutions beyond the training resolution, suggesting that the learned features capture scale-invariant matting characteristics. This multi-resolution robustness, combined with the frame-count flexibility, makes VideoMaMa a versatile tool for generating training data across diverse video scenarios.

\input{tables/ablations/stage_wise}
\paragraph{Training recipe.}
We ablate the effectiveness of our two-stage training strategy and semantic knowledge injection in YouTubeMatte~\cite{matanyone} by comparing four training configurations: (1) training only on single image (stage 1 only), (2) training only on video (stage 2 only), (3) our two-stage approach without semantic knowledge, and (4) our full model with both two-stage training and DINO semantic features. As shown in Table~\ref{tab:stage_wise}, when training exclusively on image datasets without stage 2, its output lacks temporal consistency across video sequences, resulting in degraded quantitative performance on video benchmarks. 
% \jl{delete this? The temporal inconsistency manifests as flickering artifacts and abrupt changes in alpha values between consecutive frames.} 
Conversely, when training only on video datasets, the model achieves temporally consistent video mattes but produces less sophisticated spatial details. 
% \jl{delete this? compared to our two-stage approach. This suggests that high-resolution image training is crucial for learning fine-grained matting details, while video training is essential for temporal coherence.}
Our two-stage strategy effectively combines both advantages: stage 1 training on high-resolution images captures pixel-level precision and intricate boundary details, while stage 2 training on videos ensures smooth temporal transitions and motion-aware matting. 
In addition, the result shows that adding DINO semantic features provides further improvements, particularly for videos with complex object structures and ambiguous boundaries. The semantic knowledge enables the model to better understand object categories, part relationships, and structural priors, leading to more accurate boundary localization and improved handling of challenging scenarios such as fine-grained structures and overlapping objects. 
The ablation results validate that both the two-stage training strategy and semantic knowledge injection are necessary and complementary components, with our full approach achieving the optimal balance between spatial quality, temporal consistency, and semantic understanding.

\input{tables/ablations/data_ablation_matanyone}
\input{figures/4_sam2_finetune_VS_exisiting}
\paragraph{Impact of \mbox{MA-V} dataset on matting quality.}
\label{pargraph:mav_analysis}
To further validate the quality of our \mbox{MA-V} dataset, we conduct an analysis under SAM2-Matte on different training data configurations. We evaluate the fine-tuned models on the V-HIM60~\cite{maggie} hard split, which is particularly challenging as it contains multiple object instances, allowing us to assess both matting quality and tracking performance simultaneously.

As shown in Table~\ref{tab:ablation_combined_matting_davis}, we compare three training configurations: (a) training only with existing matting datasets, (b) training only with our \mbox{MA-V} dataset, and (c) training with both existing datasets and \mbox{MA-V}. (a) achieves relatively poor performance, which can be attributed to the scarcity of existing video matting datasets and their limited diversity. Remarkably, (b), trained exclusively on \mbox{MA-V}, significantly outperforms (a) and exceeds current state-of-the-art results on the benchmark. This demonstrates that \mbox{MA-V} provides superior data quality and diversity compared to existing datasets, validating the effectiveness of our VideoMaMa generation approach.
(c), which combines existing datasets with \mbox{MA-V}, achieves the best overall performance. 
This strong performance can be attributed to the similarity between the existing datasets and V-HIM60~\cite{maggie}. The benchmark is synthetically generated by compositing multiple overlapping foreground objects, similar to the composition methodology used in existing video matting datasets. Training on these existing synthetic datasets enables our model to effectively handle V-HIM60's synthetic characteristics.

\paragraph{Impact of \mbox{MA-V} dataset on tracking capability.}
To further address the effectiveness of the \mbox{MA-V} dataset, we evaluate on DAVIS~\cite{davis} using Video Object Segmentation metrics to assess instance tracking performance on in-the-wild videos. We binarize the matting results to perform VOS evaluation.

As shown in Table~\ref{tab:ablation_combined_matting_davis}, MatAnyone~\cite{matanyone} outperforms our model trained with only existing video matting datasets (configuration a) on DAVIS, highlighting the limitations of existing video matting datasets for learning robust tracking. However, training with \mbox{MA-V}'s manually annotated data (configuration b) substantially improves performance, surpassing MatAnyone and demonstrating \mbox{MA-V}'s superior quality for learning tracking capabilities.

Interestingly, adding existing datasets to \mbox{MA-V} (configuration c) degrades tracking performance compared to training on \mbox{MA-V} alone. This suggests that existing synthetic datasets, while useful for matting quality, may introduce domain biases that harm tracking robustness on in-the-wild videos. These results validate that \mbox{MA-V} not only provides high-quality matting annotations but also enables superior tracking capabilities in real-world scenarios.

==> tables/V-HIM60.tex <==
% \begin{table*}[t]
%   \centering
%   \caption{Quantitative comparison on the \textbf{V-HIM} dataset across three difficulty levels. Green percentages denote improvement.}
%   \label{tab:vhim_comparison_final}
%   \resizebox{\textwidth}{!}{%
%   \begin{tabular}{@{}llcccccccccccc@{}}
%     \toprule
%     & & \multicolumn{4}{c}{\textbf{V-HIM (Easy)}} & \multicolumn{4}{c}{\textbf{V-HIM (Medium)}} & \multicolumn{4}{c}{\textbf{V-HIM (Hard)}} \\
%     \cmidrule(lr){3-6} \cmidrule(lr){7-10} \cmidrule(lr){11-14}
%     \textbf{Mask Style} & & \textbf{MAD} & \textbf{MAD-T} & \textbf{Grad} & \makecell{\textbf{Video Improved /} \\ \textbf{Worsen (Frame)}} & \textbf{MAD} & \textbf{MAD-T} & \textbf{Grad} & \makecell{\textbf{Video Improved /} \\ \textbf{Worsen (Frame)}} & \textbf{MAD} & \textbf{MAD-T} & \textbf{Grad} & \makecell{\textbf{Video Improved /} \\ \textbf{Worsen (Frame)}} \\
%     \midrule
%     \multirow{3}{*}{Down \& Up 8} & Before & 2.0271 & 147.9786 & 8.3479 & \multirow{3}{*}{45 (531) / 2 (28)} & 3.0836 & 143.1936 & 12.5451 & \multirow{3}{*}{43 (510) / 0 (0)} & 2.7442 & 147.3277 & 11.1271 & \multirow{3}{*}{53 (632) / 1 (13)} \\
%     & Refined & 0.9946 & 67.3905 & 2.2579 & & 1.3839 & 60.9983 & 2.6235 & & 1.3057 & 62.2222 & 2.3628 & \\
%     & Improvement & \textcolor{green!70!black}{50.93\%} & \textcolor{green!70!black}{54.46\%} & \textcolor{green!70!black}{72.95\%} & & \textcolor{green!70!black}{55.12\%} & \textcolor{green!70!black}{57.40\%} & \textcolor{green!70!black}{79.09\%} & & \textcolor{green!70!black}{52.42\%} & \textcolor{green!70!black}{57.77\%} & \textcolor{green!70!black}{78.77\%} & \\
%     \midrule
%     \multirow{3}{*}{Down \& Up 32} & Before & 3.8209 & 249.3027 & 26.9541 & \multirow{3}{*}{47 (557) / 0 (2)} & 5.8671 & 247.6536 & 41.0621 & \multirow{3}{*}{43 (510) / 0 (0)} & 5.1316 & 241.6574 & 33.6640 & \multirow{3}{*}{54 (644) / 0 (1)} \\
%     & Refined & 1.0564 & 70.9592 & 2.4617 & & 1.5295 & 66.2501 & 3.2285 & & 1.4608 & 68.4286 & 2.8492 & \\
%     & Improvement & \textcolor{green!70!black}{72.35\%} & \textcolor{green!70!black}{71.54\%} & \textcolor{green!70!black}{90.87\%} & & \textcolor{green!70!black}{73.93\%} & \textcolor{green!70!black}{73.25\%} & \textcolor{green!70!black}{92.14\%} & & \textcolor{green!70!black}{71.53\%} & \textcolor{green!70!black}{71.68\%} & \textcolor{green!70!black}{91.54\%} & \\
%     \midrule
%     \multirow{3}{*}{Polygon (Easy)} & Before & 2.6845 & 167.1927 & 12.2152 & \multirow{3}{*}{47 (550) / 0 (9)} & 4.5873 & 172.6466 & 21.3605 & \multirow{3}{*}{43 (510) / 0 (0)} & 3.6361 & 162.5674 & 15.9996 & \multirow{3}{*}{53 (632) / 1 (13)} \\
%     & Refined & 1.0293 & 68.4758 & 2.2954 & & 1.5284 & 63.9046 & 2.9710 & & 1.4157 & 63.5057 & 2.4799 & \\
%     & Improvement & \textcolor{green!70!black}{61.66\%} & \textcolor{green!70!black}{59.04\%} & \textcolor{green!70!black}{81.21\%} & & \textcolor{green!70!black}{66.68\%} & \textcolor{green!70!black}{62.99\%} & \textcolor{green!70!black}{86.09\%} & & \textcolor{green!70!black}{61.06\%} & \textcolor{green!70!black}{60.94\%} & \textcolor{green!70!black}{84.50\%} & \\
%     \midrule
%     \multirow{3}{*}{Polygon (Hard)} & Before & 5.0768 & 273.1866 & 35.8950 & \multirow{3}{*}{47 (557) / 0 (2)} & 9.4215 & 287.3694 & 60.0112 & \multirow{3}{*}{43 (510) / 0 (0)} & 6.7708 & 252.4623 & 43.2282 & \multirow{3}{*}{54 (644) / 0 (1)} \\
%     & Refined & 1.1181 & 72.2534 & 2.5582 & & 1.7910 & 68.5288 & 3.6736 & & 1.6403 & 68.3408 & 3.0243 & \\
%     & Improvement & \textcolor{green!70!black}{77.98\%} & \textcolor{green!70!black}{73.55\%} & \textcolor{green!70!black}{92.87\%} & & \textcolor{green!70!black}{80.99\%} & \textcolor{green!70!black}{76.15\%} & \textcolor{green!70!black}{93.88\%} & & \textcolor{green!70!black}{75.77\%} & \textcolor{green!70!black}{72.93\%} & \textcolor{green!70!black}{93.00\%} & \\
%     \midrule
%     \multirow{3}{*}{Point 5} & Before & 4.5022 & 195.3625 & 13.9393 & \multirow{3}{*}{46 (540) / 1 (19)} & 4.8094 & 193.2853 & 24.6467 & \multirow{3}{*}{43 (510) / 0 (0)} & 4.6658 & 195.8977 & 21.9602 & \multirow{3}{*}{53 (638) / 1 (7)} \\
%     & Refined & 3.1245 & 93.1978 & 3.6781 & & 2.2470 & 74.6025 & 4.3417 & & 2.4350 & 78.9677 & 4.1802 & \\
%     & Improvement & \textcolor{green!70!black}{30.60\%} & \textcolor{green!70!black}{52.29\%} & \textcolor{green!70!black}{73.61\%} & & \textcolor{green!70!black}{53.28\%} & \textcolor{green!70!black}{61.40\%} & \textcolor{green!70!black}{82.38\%} & & \textcolor{green!70!black}{47.81\%} & \textcolor{green!70!black}{59.69\%} & \textcolor{green!70!black}{80.96\%} & \\
%     \midrule
%     \multirow{3}{*}{MatAnyone} & Before & 3.1734 & 149.7782 & 6.4559 & \multirow{3}{*}{39 (481) / 8 (78)} & 5.9308 & 156.0849 & 10.4775 & \multirow{3}{*}{43 (503) / 0 (7)} & 4.6655 & 163.1032 & 8.8870 & \multirow{3}{*}{53 (608) / 1 (37)} \\
%     & Refined & 2.0199 & 95.4806 & 3.4797 & & 3.6929 & 87.5698 & 4.8894 & & 3.1020 & 101.4569 & 4.7492 & \\
%     & Improvement & \textcolor{green!70!black}{36.35\%} & \textcolor{green!70!black}{36.25\%} & \textcolor{green!70!black}{46.10\%} & & \textcolor{green!70!black}{37.73\%} & \textcolor{green!70!black}{43.90\%} & \textcolor{green!70!black}{53.33\%} & & \textcolor{green!70!black}{33.51\%} & \textcolor{green!70!black}{37.80\%} & \textcolor{green!70!black}{46.56\%} & \\
%     \midrule
%     \multirow{3}{*}{MaGGle} & Before & 1.9705 & 105.9294 & 4.1788 & \multirow{3}{*}{41 (477) / 6 (82)} & 3.2311 & 105.2581 & 6.8928 & \multirow{3}{*}{41 (489) / 2 (21)} & 3.6835 & 109.0113 & 6.5221 & \multirow{3}{*}{53 (622) / 1 (23)} \\
%     & Refined & 1.3318 & 74.7918 & 2.7673 & & 1.9982 & 71.7087 & 3.9026 & & 2.4371 & 75.5989 & 3.8445 & \\
%     & Improvement & \textcolor{green!70!black}{32.41\%} & \textcolor{green!70!black}{29.39\%} & \textcolor{green!70!black}{33.78\%} & & \textcolor{green!70!black}{38.16\%} & \textcolor{green!70!black}{31.87\%} & \textcolor{green!70!black}{43.38\%} & & \textcolor{green!70!black}{33.84\%} & \textcolor{green!70!black}{30.65\%} & \textcolor{green!70!black}{41.05\%} & \\
%     \midrule
%     \multirow{3}{*}{GT Mask Guided} & Before & 7.8823 & 297.0182 & 40.8435 & \multirow{3}{*}{46 (524) / 1 (35)} & 11.8469 & 299.6511 & 62.5424 & \multirow{3}{*}{43 (497) / 0 (13)} & 10.4643 & 293.8532 & 51.7756 & \multirow{3}{*}{54 (630) / 0 (15)} \\
%     & Refined & 1.9090 & 89.4316 & 3.2971 & & 2.3360 & 78.7730 & 3.8238 & & 2.3403 & 84.8793 & 3.7752 & \\
%     & Improvement & \textcolor{green!70!black}{75.78\%} & \textcolor{green!70!black}{69.89\%} & \textcolor{green!70!black}{91.93\%} & & \textcolor{green!70!black}{80.28\%} & \textcolor{green!70!black}{73.71\%} & \textcolor{green!70!black}{93.89\%} & & \textcolor{green!70!black}{77.64\%} & \textcolor{green!70!black}{71.12\%} & \textcolor{green!70!black}{92.71\%} & \\
%     \bottomrule
%   \end{tabular}
%   } % end \resizebox
% \end{table*}

\begin{table*}[h]
  \centering
  \resizebox{\textwidth}{!}{%
  \begin{tabular}{@{}lcccccccccccccccccc@{}}
    \toprule
    & \multicolumn{6}{c}{\textbf{Easy}} & \multicolumn{6}{c}{\textbf{Medium}} & \multicolumn{6}{c}{\textbf{Hard}} \\
    \cmidrule(lr){2-7} \cmidrule(lr){8-13} \cmidrule(lr){14-19}
    & \multicolumn{3}{c}{MAD $\downarrow$} & \multicolumn{3}{c}{Gradient $\downarrow$} & \multicolumn{3}{c}{MAD $\downarrow$} & \multicolumn{3}{c}{Gradient $\downarrow$} & \multicolumn{3}{c}{MAD $\downarrow$} & \multicolumn{3}{c}{Gradient $\downarrow$} \\
    \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13} \cmidrule(lr){14-16} \cmidrule(lr){17-19}
    \textbf{Mask Type} & Init & Ref & $\Delta$ & Init & Ref & $\Delta$ & Init & Ref & $\Delta$ & Init & Ref & $\Delta$ & Init & Ref & $\Delta$ & Init & Ref & $\Delta$ \\
    \midrule
    D\&U 8        & 2.027 & 0.995 & \textcolor{green!70!black}{50.9\%} & 8.348 & 2.258 & \textcolor{green!70!black}{73.0\%} & 3.084 & 1.384 & \textcolor{green!70!black}{55.1\%} & 12.545 & 2.624 & \textcolor{green!70!black}{79.1\%} & 2.744 & 1.306 & \textcolor{green!70!black}{52.4\%} & 11.127 & 2.363 & \textcolor{green!70!black}{78.8\%} \\
    D\&U 32       & 3.821 & 1.056 & \textcolor{green!70!black}{72.4\%} & 26.954 & 2.462 & \textcolor{green!70!black}{90.9\%} & 5.867 & 1.530 & \textcolor{green!70!black}{73.9\%} & 41.062 & 3.229 & \textcolor{green!70!black}{92.1\%} & 5.132 & 1.461 & \textcolor{green!70!black}{71.5\%} & 33.664 & 2.849 & \textcolor{green!70!black}{91.5\%} \\
    Poly(E)       & 2.685 & 1.029 & \textcolor{green!70!black}{61.7\%} & 12.215 & 2.295 & \textcolor{green!70!black}{81.2\%} & 4.587 & 1.528 & \textcolor{green!70!black}{66.7\%} & 21.361 & 2.971 & \textcolor{green!70!black}{86.1\%} & 3.636 & 1.416 & \textcolor{green!70!black}{61.1\%} & 16.000 & 2.480 & \textcolor{green!70!black}{84.5\%} \\
    Poly(H)       & 5.077 & 1.118 & \textcolor{green!70!black}{78.0\%} & 35.895 & 2.558 & \textcolor{green!70!black}{92.9\%} & 9.422 & 1.791 & \textcolor{green!70!black}{81.0\%} & 60.011 & 3.674 & \textcolor{green!70!black}{93.9\%} & 6.771 & 1.640 & \textcolor{green!70!black}{75.8\%} & 43.228 & 3.024 & \textcolor{green!70!black}{93.0\%} \\
    SAM2~\cite{sam2}       & 4.502 & 3.125 & \textcolor{green!70!black}{30.6\%} & 13.939 & 3.678 & \textcolor{green!70!black}{73.6\%} & 4.809 & 2.247 & \textcolor{green!70!black}{53.3\%} & 24.647 & 4.342 & \textcolor{green!70!black}{82.4\%} & 4.666 & 2.435 & \textcolor{green!70!black}{47.8\%} & 21.960 & 4.180 & \textcolor{green!70!black}{81.0\%} \\
    MatAnyone~\cite{matanyone}     & 3.173 & 2.020 & \textcolor{green!70!black}{36.4\%} & 6.456 & 3.480 & \textcolor{green!70!black}{46.1\%} & 5.931 & 3.693 & \textcolor{green!70!black}{37.7\%} & 10.478 & 4.889 & \textcolor{green!70!black}{53.3\%} & 4.666 & 3.102 & \textcolor{green!70!black}{33.5\%} & 8.887 & 4.749 & \textcolor{green!70!black}{46.6\%} \\
    MaGGle~\cite{maggie}        & 1.971 & 1.332 & \textcolor{green!70!black}{32.4\%} & 4.179 & 2.767 & \textcolor{green!70!black}{33.8\%} & 3.231 & 1.998 & \textcolor{green!70!black}{38.2\%} & 6.893 & 3.903 & \textcolor{green!70!black}{43.4\%} & 3.684 & 2.437 & \textcolor{green!70!black}{33.8\%} & 6.522 & 3.845 & \textcolor{green!70!black}{41.1\%} \\
    XMem~\cite{xmem}     & 7.882 & 1.909 & \textcolor{green!70!black}{75.8\%} & 40.844 & 3.297 & \textcolor{green!70!black}{91.9\%} & 11.847 & 2.336 & \textcolor{green!70!black}{80.3\%} & 62.542 & 3.824 & \textcolor{green!70!black}{93.9\%} & 10.464 & 2.340 & \textcolor{green!70!black}{77.6\%} & 51.776 & 3.775 & \textcolor{green!70!black}{92.7\%} \\
    \bottomrule
  \end{tabular}
  }
  \caption{Mask-to-matte refinement results on V-HIM dataset~\cite{maggie} across three difficulty levels. For each metric, we show Initial mask quality / Refined quality / Improvement(\%). D\&U: Down \& Upsampling. Poly(E/H): Polygon Easy/Hard. MAD: Mean Absolute Difference. Lower is better for all metrics.}
  \label{tab:vhim_refinement}
\end{table*}

==> tables/VideoMatte.tex <==
% \begin{table*}[t]
%   \centering
%   \caption{Quantitative comparison of different mask styles before and after refinement. We evaluate on two resolutions using Mean Absolute Difference (MAD), MAD with temporal coherence (MAD-T), and Gradient (Grad) metrics. Lower values are better for all metrics. The percentage improvement is shown in the third row for each style; positive improvements are colored green.}
%   \label{tab:mask_style_comparison_merged}
%   \resizebox{\textwidth}{!}{%
%   \begin{tabular}{@{}llcccccccc@{}}
%     \toprule
%     & & \multicolumn{4}{c}{\textbf{VideoMatte (512 x 288)}} & \multicolumn{4}{c}{\textbf{VideoMatte (1920 x 1080)}} \\
%     \cmidrule(lr){3-6} \cmidrule(lr){7-10}
%     \textbf{Mask Style} & & \textbf{MAD} & \textbf{MAD-T} & \textbf{Grad} & \makecell{\textbf{Video Improved /} \\ \textbf{Worsen (Frame)}} & \textbf{MAD} & \textbf{MAD-T} & \textbf{Grad} & \makecell{\textbf{Video Improved /} \\ \textbf{Worsen (Frame)}} \\
%     \midrule
%     \multirow{3}{*}{Down \& Up 8} & Before & 5.2667 & 6.4127 & 0.1850 & \multirow{3}{*}{50 (598) / 0 (2)} & 4.7447 & 5.7960 & 6.5277 & \multirow{3}{*}{50 (600) / 0 (0)} \\
%     & Refined & 4.1246 & 4.9571 & 0.0785 & & 3.8159 & 4.6200 & 1.5703 & \\
%     & Improvement & \textcolor{green!70!black}{21.68\%} & \textcolor{green!70!black}{22.70\%} & \textcolor{green!70!black}{57.58\%} & & \textcolor{green!70!black}{19.58\%} & \textcolor{green!70!black}{20.29\%} & \textcolor{green!70!black}{75.94\%} & \\
%     \midrule
%     \multirow{3}{*}{Down \& Up 32} & Before & 8.0347 & 9.3096 & 3.0011 & \multirow{3}{*}{50 (600) / 0 (0)} & 7.8437 & 8.5028 & 44.4962 & \multirow{3}{*}{50 (600) / 0 (0)} \\
%     & Refined & 4.2551 & 5.0708 & 0.1385 & & 3.8837 & 4.6708 & 2.0505 & \\
%     & Improvement & \textcolor{green!70!black}{47.04\%} & \textcolor{green!70!black}{45.53\%} & \textcolor{green!70!black}{95.39\%} & & \textcolor{green!70!black}{50.49\%} & \textcolor{green!70!black}{45.07\%} & \textcolor{green!70!black}{95.39\%} & \\
%     \midrule
%     \multirow{3}{*}{Polygon (Easy)} & Before & 5.8825 & 7.1566 & 0.6747 & \multirow{3}{*}{50 (600) / 0 (0)} & 5.5603 & 6.6613 & 17.5452 & \multirow{3}{*}{50 (600) / 0 (0)} \\
%     & Refined & 4.1553 & 4.9881 & 0.0917 & & 3.8337 & 4.6346 & 1.6004 & \\
%     & Improvement & \textcolor{green!70!black}{29.36\%} & \textcolor{green!70!black}{30.30\%} & \textcolor{green!70!black}{86.40\%} & & \textcolor{green!70!black}{31.05\%} & \textcolor{green!70!black}{30.42\%} & \textcolor{green!70!black}{90.88\%} & \\
%     \midrule
%     \multirow{3}{*}{Polygon (Hard)} & Before & 11.2386 & 11.9081 & 7.1671 & \multirow{3}{*}{50 (600) / 0 (0)} & 11.2595 & 10.6837 & 67.9442 & \multirow{3}{*}{50 (600) / 0 (0)} \\
%     & Refined & 4.3826 & 5.1748 & 0.1905 & & 3.9517 & 4.7235 & 2.2056 & \\
%     & Improvement & \textcolor{green!70!black}{61.00\%} & \textcolor{green!70!black}{56.54\%} & \textcolor{green!70!black}{97.34\%} & & \textcolor{green!70!black}{64.90\%} & \textcolor{green!70!black}{55.79\%} & \textcolor{green!70!black}{96.75\%} & \\
%     \midrule
%     \multirow{3}{*}{SAM2 (Point 5)} & Before & 6.7087 & 7.5346 & 0.8997 & \multirow{3}{*}{50 (600) / 0 (0)} & 5.3068 & 6.3256 & 14.5117 & \multirow{3}{*}{50 (600) / 0 (0)} \\
%     & Refined & 4.8466 & 5.1827 & 0.3164 & & 4.0343 & 4.7668 & 2.6527 & \\
%     & Improvement & \textcolor{green!70!black}{27.76\%} & \textcolor{green!70!black}{31.22\%} & \textcolor{green!70!black}{64.83\%} & & \textcolor{green!70!black}{23.98\%} & \textcolor{green!70!black}{24.64\%} & \textcolor{green!70!black}{81.72\%} & \\
%     \midrule
%     \multirow{3}{*}{MatAnyone (Reproduce)} & Before & 4.6061 & 5.4865 & 0.4302 & \multirow{3}{*}{40 (477) / 10 (123)} & 4.3267 & 5.1464 & 4.2006 & \multirow{3}{*}{50 (600) / 0 (0)} \\
%     & Refined & 4.3105 & 5.1360 & 0.1801 & & 3.9181 & 4.7218 & 2.1162 & \\
%     & Improvement & \textcolor{green!70!black}{6.42\%} & \textcolor{green!70!black}{6.39\%} & \textcolor{green!70!black}{58.14\%} & & \textcolor{green!70!black}{9.44\%} & \textcolor{green!70!black}{8.25\%} & \textcolor{green!70!black}{49.62\%} & \\
%     \bottomrule
%   \end{tabular}
%   } % end \resizebox
% \end{table*}

\begin{table*}[t]
  \centering
  \resizebox{\textwidth}{!}{%
  \begin{tabular}{@{}lcccccccccccc@{}}
    \toprule
    & \multicolumn{6}{c}{\textbf{512 $\times$ 288}} & \multicolumn{6}{c}{\textbf{1920 $\times$ 1080}} \\
    \cmidrule(lr){2-7} \cmidrule(lr){8-13}
    & \multicolumn{3}{c}{MAD $\downarrow$} & \multicolumn{3}{c}{Gradient $\downarrow$} & \multicolumn{3}{c}{MAD $\downarrow$} & \multicolumn{3}{c}{Gradient $\downarrow$} \\
    \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13}
    \textbf{Mask Type} & Init & Ref & $\Delta$ & Init & Ref & $\Delta$ & Init & Ref & $\Delta$ & Init & Ref & $\Delta$ \\
    \midrule
    D\&U 8             & 5.267 & 4.125 & \textcolor{green!70!black}{21.7\%} & 0.185 & 0.079 & \textcolor{green!70!black}{57.6\%} & 4.745 & 3.816 & \textcolor{green!70!black}{19.6\%} & 6.528 & 1.570 & \textcolor{green!70!black}{75.9\%} \\
    D\&U 32            & 8.035 & 4.255 & \textcolor{green!70!black}{47.0\%} & 3.001 & 0.139 & \textcolor{green!70!black}{95.4\%} & 7.844 & 3.884 & \textcolor{green!70!black}{50.5\%} & 44.496 & 2.051 & \textcolor{green!70!black}{95.4\%} \\
    Poly(E)            & 5.883 & 4.155 & \textcolor{green!70!black}{29.4\%} & 0.675 & 0.092 & \textcolor{green!70!black}{86.4\%} & 5.560 & 3.834 & \textcolor{green!70!black}{31.1\%} & 17.545 & 1.600 & \textcolor{green!70!black}{90.9\%} \\
    Poly(H)            & 11.239 & 4.383 & \textcolor{green!70!black}{61.0\%} & 7.167 & 0.191 & \textcolor{green!70!black}{97.3\%} & 11.260 & 3.952 & \textcolor{green!70!black}{64.9\%} & 67.944 & 2.206 & \textcolor{green!70!black}{96.8\%} \\
    SAM2~\cite{sam2}      & 6.709 & 4.847 & \textcolor{green!70!black}{27.8\%} & 0.900 & 0.316 & \textcolor{green!70!black}{64.8\%} & 5.307 & 4.034 & \textcolor{green!70!black}{24.0\%} & 14.512 & 2.653 & \textcolor{green!70!black}{81.7\%} \\
    MatAnyone~\cite{matanyone}  & 4.606 & 4.311 & \textcolor{green!70!black}{6.4\%} & 0.430 & 0.180 & \textcolor{green!70!black}{58.1\%} & 4.327 & 3.918 & \textcolor{green!70!black}{9.4\%} & 4.201 & 2.116 & \textcolor{green!70!black}{49.6\%} \\
    \bottomrule
  \end{tabular}
  }
  \caption{Mask-to-matte refinement results on VideoMatte dataset~\cite{video240k} at two resolutions. For each metric, we show Initial mask quality / Refined quality / Improvement(\%). D\&U: Down \& Upsampling. Poly(E/H): Polygon Easy/Hard. MAD: Mean Absolute Difference. Repro: Reproduced. Lower is better for all metrics.}
  \label{tab:videomatte_refined}
\end{table*}

==> tables/YouTubeMatte.tex <==
% \begin{table*}[t]
%   \centering
%   \caption{Quantitative comparison on the \textbf{YouTubeMatte} dataset. Green percentages denote improvement.}
%   \label{tab:youtubematte_corrected_full}
%   \resizebox{\textwidth}{!}{%
%   \begin{tabular}{@{}llcccccccc@{}}
%     \toprule
%     & & \multicolumn{4}{c}{\textbf{512 x 288 (Static + Motion)}} & \multicolumn{4}{c}{\textbf{1920 x 1080 (Static + Motion)}} \\
%     \cmidrule(lr){3-6} \cmidrule(lr){7-10}
%     \textbf{Mask Style} & & \textbf{MAD} & \textbf{MAD-T} & \textbf{Grad} & \makecell{\textbf{Video Improved /} \\ \textbf{Worsen (Frame)}} & \textbf{MAD} & \textbf{MAD-T} & \textbf{Grad} & \makecell{\textbf{Video Improved /} \\ \textbf{Worsen (Frame)}} \\
%     \midrule
%     \multirow{3}{*}{Down \& Up 8} & Before & 1.9204 & 83.4015 & 0.1661 & \multirow{3}{*}{61 (724) / 3 (44)} & 1.9460 & 128.3496 & 8.0343 & \multirow{3}{*}{64 (768) / 0 (0)} \\
%     & Refined & 1.4889 & 48.1579 & 0.1107 & & 0.9340 & 55.2653 & 2.0313 & \\
%     & Improvement & \textcolor{green!70!black}{22.47\%} & \textcolor{green!70!black}{42.26\%} & \textcolor{green!70!black}{33.30\%} & & \textcolor{green!70!black}{52.01\%} & \textcolor{green!70!black}{56.94\%} & \textcolor{green!70!black}{74.72\%} & \\
%     \midrule
%     \multirow{3}{*}{Down \& Up 32} & Before & 4.1669 & 155.1671 & 2.2766 & \multirow{3}{*}{64 (768) / 0 (0)} & 4.2029 & 225.2391 & 36.5395 & \multirow{3}{*}{64 (768) / 0 (0)} \\
%     & Refined & 1.6257 & 52.2738 & 0.1911 & & 1.0292 & 59.8396 & 2.5602 & \\
%     & Improvement & \textcolor{green!70!black}{60.98\%} & \textcolor{green!70!black}{66.31\%} & \textcolor{green!70!black}{91.60\%} & & \textcolor{green!70!black}{75.51\%} & \textcolor{green!70!black}{73.43\%} & \textcolor{green!70!black}{92.99\%} & \\
%     \midrule
%     \multirow{3}{*}{Polygon (Easy)} & Before & 3.5976 & 112.6883 & 0.9816 & \multirow{3}{*}{64 (768) / 0 (0)} & 3.6190 & 164.3361 & 19.1551 & \multirow{3}{*}{64 (768) / 0 (0)} \\
%     & Refined & 1.7176 & 50.3130 & 0.1672 & & 1.2056 & 57.7615 & 2.3350 & \\
%     & Improvement & \textcolor{green!70!black}{52.26\%} & \textcolor{green!70!black}{55.35\%} & \textcolor{green!70!black}{82.97\%} & & \textcolor{green!70!black}{66.69\%} & \textcolor{green!70!black}{64.85\%} & \textcolor{green!70!black}{87.81\%} & \\
%     \midrule
%     \multirow{3}{*}{Polygon (Hard)} & Before & 9.3813 & 247.5662 & 7.8246 & \multirow{3}{*}{64 (768) / 0 (0)} & 9.4700 & 337.2268 & 65.8438 & \multirow{3}{*}{64 (768) / 0 (0)} \\
%     & Refined & 2.0152 & 57.3483 & 0.2722 & & 1.4042 & 65.9612 & 3.2374 & \\
%     & Improvement & \textcolor{green!70!black}{78.51\%} & \textcolor{green!70!black}{76.84\%} & \textcolor{green!70!black}{96.52\%} & & \textcolor{green!70!black}{85.17\%} & \textcolor{green!70!black}{80.44\%} & \textcolor{green!70!black}{95.08\%} & \\
%     \midrule
%     \multirow{3}{*}{Point 5} & Before & 5.0479 & 141.7661 & 1.5833 & \multirow{3}{*}{64 (768) / 0 (0)} & 3.5693 & 181.0797 & 24.7291 & \multirow{3}{*}{64 (768) / 0 (0)} \\
%     & Refined & 3.3678 & 59.5790 & 0.5023 & & 1.7370 & 65.5267 & 3.6353 & \\
%     & Improvement & \textcolor{green!70!black}{33.28\%} & \textcolor{green!70!black}{57.97\%} & \textcolor{green!70!black}{68.27\%} & & \textcolor{green!70!black}{51.33\%} & \textcolor{green!70!black}{63.81\%} & \textcolor{green!70!black}{85.30\%} & \\
%     \midrule
%     \multirow{3}{*}{MatAnyone (Reproduce)} & Before & 2.5011 & 82.9218 & 0.8136 & \multirow{3}{*}{60 (713) / 4 (55)} & 1.7971 & 96.0814 & 6.8380 & \multirow{3}{*}{64 (767) / 0 (1)} \\
%     & Refined & 1.7273 & 54.4347 & 0.2531 & & 1.0707 & 62.0975 & 2.6959 & \\
%     & Improvement & \textcolor{green!70!black}{30.94\%} & \textcolor{green!70!black}{34.35\%} & \textcolor{green!70!black}{68.89\%} & & \textcolor{green!70!black}{40.42\%} & \textcolor{green!70!black}{35.37\%} & \textcolor{green!70!black}{60.58\%} & \\
%     \midrule
%     \multirow{3}{*}{Matanyone} & Before & 2.73185 & 87.8902 & 0.9823 & \multirow{3}{*}{60 (728) / 4 (40)} & 2.2191 & 121.9952 & 10.2171 & \multirow{3}{*}{64 (767) / 0 (1)} \\
%     & Refined & 1.8743 & 56.3978 & 0.3206 & & 1.2807 & 65.5474 & 3.1492 & \\
%     & Improvement & \textcolor{green!70!black}{31.39\%} & \textcolor{green!70!black}{35.83\%} & \textcolor{green!70!black}{67.36\%} & & \textcolor{green!70!black}{42.29\%} & \textcolor{green!70!black}{46.27\%} & \textcolor{green!70!black}{69.18\%} & \\
%     \bottomrule
%   \end{tabular}
%   } % end \resizebox
% \end{table*}

\begin{table*}[t]
  \centering
  \resizebox{\textwidth}{!}{%
  \begin{tabular}{@{}lcccccccccccc@{}}
    \toprule
    & \multicolumn{6}{c}{\textbf{512 $\times$ 288}} & \multicolumn{6}{c}{\textbf{1920 $\times$ 1080}} \\
    \cmidrule(lr){2-7} \cmidrule(lr){8-13}
    & \multicolumn{3}{c}{MAD $\downarrow$} & \multicolumn{3}{c}{Gradient $\downarrow$} & \multicolumn{3}{c}{MAD $\downarrow$} & \multicolumn{3}{c}{Gradient $\downarrow$} \\
    \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13}
    \textbf{Mask Type} & Init & Ref & $\Delta$ & Init & Ref & $\Delta$ & Init & Ref & $\Delta$ & Init & Ref & $\Delta$ \\
    \midrule
    D\&U 8             & 1.920 & 1.489 & \textcolor{green!70!black}{22.5\%} & 0.166 & 0.111 & \textcolor{green!70!black}{33.3\%} & 1.946 & 0.934 & \textcolor{green!70!black}{52.0\%} & 8.034 & 2.031 & \textcolor{green!70!black}{74.7\%} \\
    D\&U 32            & 4.167 & 1.626 & \textcolor{green!70!black}{61.0\%} & 2.277 & 0.191 & \textcolor{green!70!black}{91.6\%} & 4.203 & 1.029 & \textcolor{green!70!black}{75.5\%} & 36.540 & 2.560 & \textcolor{green!70!black}{93.0\%} \\
    Poly(E)            & 3.598 & 1.718 & \textcolor{green!70!black}{52.3\%} & 0.982 & 0.167 & \textcolor{green!70!black}{83.0\%} & 3.619 & 1.206 & \textcolor{green!70!black}{66.7\%} & 19.155 & 2.335 & \textcolor{green!70!black}{87.8\%} \\
    Poly(H)            & 9.381 & 2.015 & \textcolor{green!70!black}{78.5\%} & 7.825 & 0.272 & \textcolor{green!70!black}{96.5\%} & 9.470 & 1.404 & \textcolor{green!70!black}{85.2\%} & 65.844 & 3.237 & \textcolor{green!70!black}{95.1\%} \\
    SAM2~\cite{sam2}            & 5.048 & 3.368 & \textcolor{green!70!black}{33.3\%} & 1.583 & 0.502 & \textcolor{green!70!black}{68.3\%} & 3.569 & 1.737 & \textcolor{green!70!black}{51.3\%} & 24.729 & 3.635 & \textcolor{green!70!black}{85.3\%} \\
    MatAnyone~\cite{matanyone} (Repro)  & 2.501 & 1.727 & \textcolor{green!70!black}{30.9\%} & 0.814 & 0.253 & \textcolor{green!70!black}{68.9\%} & 1.797 & 1.071 & \textcolor{green!70!black}{40.4\%} & 6.838 & 2.696 & \textcolor{green!70!black}{60.6\%} \\
    MatAnyone          & 2.732 & 1.874 & \textcolor{green!70!black}{31.4\%} & 0.982 & 0.321 & \textcolor{green!70!black}{67.4\%} & 2.219 & 1.281 & \textcolor{green!70!black}{42.3\%} & 10.217 & 3.149 & \textcolor{green!70!black}{69.2\%} \\
    \bottomrule
  \end{tabular}
  }
  \caption{Mask-to-matte refinement results on YouTubeMatte dataset~\cite{matanyone} at two resolutions (Static + Motion). For each metric, we show Initial mask quality / Refined quality / Improvement(\%). D\&U: Down \& Upsampling. Poly(E/H): Polygon Easy/Hard. MAD: Mean Absolute Difference. Repro: Reproduced. Lower is better for all metrics.}
  \label{tab:youtubematte_refined}
\end{table*}

==> tables/ablations/sam2_vhim60_hard.tex <==
\begin{table}[t]
 \centering
 % Resize the tabular environment to fit the column width
 \resizebox{\columnwidth}{!}{%
 % Removed MAV and External Dataset columns (was l c c | c c c c c c)
 \begin{tabular}{l c c c c c c}
 \toprule
 % Removed MAV and External Dataset from header
 \textbf{Method} & \textbf{MAD} & \textbf{MAD-T} & \textbf{MSE} & \textbf{GRAD} & \textbf{CONN} & \textbf{DTSSD} \\
 \midrule
 % --- Maggie Row ---
 % Renamed from 'MaGGIe (origin)' and removed other MaGGIe rows
 MaGGIe & 3.9342 & 111.8249 & 2.0322 & 7.0463 & 6.8843 & 4.0141 \\
 % --- ADDED MatAnyone ROW ---
 MatAnyone & 4.6655 & 163.1032 & 2.5870 & 8.8870 & 8.6553 & 4.2970 \\

 \midrule % The midline

 % --- Our Results ---
 % (a) - Renamed from SAM2
 (a) ED & 7.5798 & 124.8251 & 5.6824 & 8.7091 & 14.4237 & 3.7045 \\
 (b) Manual & 3.1830 & 107.4493 & 1.5603 & 5.7869 & 5.5579 & 3.0781 \\
 (c) Auto+Manual+ED & 2.6085 & 102.29 & 1.0423 & 5.2366 & 4.4827 & 2.8158 \\

 \bottomrule
 \end{tabular}
 } % End of \resizebox
 % Updated caption
 \caption{Ablation study results. ED denotes existing dataset.}
 \label{tab:my_ablation_revised}
\end{table}

==> tables/ablations/tracking_tracking.tex <==
\begin{table}[h]
\centering
% \resizebox will force the table to fit the column width.
% Note: This table now has 10 data columns instead of 9.
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l
                S[table-format=2.1]
                S[table-format=2.1]
                S[table-format=2.1]
                S[table-format=2.1]
                S[table-format=2.1]
                S[table-format=2.1]
                S[table-format=2.1]
                S[table-format=2.1]
                S[table-format=2.1]
                S[table-format=2.1]}
\toprule
% Headers now have 5 columns per dataset
\multirow{2}{*}{\textbf{Method}} & \multicolumn{5}{c}{\textbf{DAVIS}} & \multicolumn{5}{c}{\textbf{SAV}} \\
% Partial rules adjusted for 5 columns
\cmidrule(lr){2-6} \cmidrule(lr){7-11}
% New metric sub-headers
& {HOTA} & {DetA} & {AssA} & {IDF1} & {MOTA} & {HOTA} & {DetA} & {AssA} & {IDF1} & {MOTA} \\
\midrule
% --- Baselines ---
\multicolumn{11}{l}{\textit{Baselines}} \\
% SAM2 scores updated for DAVIS (from prev) and SAV (new), all bolded
SAM2         & \textbf{94.5} & \textbf{94.8} & \textbf{94.3} & \textbf{96.4} & \textbf{93.0} & \textbf{74.6} & \textbf{77.7} & \textbf{71.9} & \textbf{81.2} & \textbf{66.5} \\
% Matanyone scores added for DAVIS (from prev) and SAV (new)
Matanyone    & 89.5 & 89.9 & 89.1 & 92.9 & 86.5 & 33.8 & 39.8 & 30.2 & 40.4 & -2.3 \\
\midrule
% --- Your Method + Ablations (New Order) ---
\multicolumn{11}{l}{\textit{Our Method (Ablations)}} \\
% (a) w/o MAV scores updated for DAVIS (from prev) and SAV (new)
(a) w/o MAV & 82.7 & 83.7 & 81.7 & 87.4 & 75.8 & 35.0 & 40.0 & 31.7 & 42.2 & -15.5 \\
% (b) Only Manual scores updated for DAVIS (from prev) and SAV (new)
(b) Only Manual & 92.5 & 92.8 & 92.1 & 95.0 & 90.3 & 54.9 & 59.5 & 51.2 & 63.1 & 20.4 \\
% (c) Manual+ED scores updated for DAVIS (from prev) and SAV (new)
(c) Manual+ED & 91.8 & 92.1 & 91.5 & 94.5 & 89.3 & 58.5 & 62.8 & 55.0 & 66.4 & 31.5 \\
% (d) Auto+Manual+ED scores updated for DAVIS (from prev) and SAV (new)
(d) Auto+Manual+ED & 92.4 & 92.7 & 92.1 & 95.0 & 90.2 & 61.0 & 65.2 & 57.7 & 68.6 & 41.6 \\
\bottomrule
\end{tabular}%
} % End of \resizebox
\caption{
    % Updated caption: removed 1080p, changed metrics, and fixed ablation list
    Quantitative ablation on DAVIS val \& SAV val.
    We report HOTA, DetA, AssA, IDF1, and MOTA. Best in \textbf{bold}.
    Our ablations: (a) w/o MAV, (b) Only Manual, (c) Manual+ED, (d) Auto+Manual+ED.
}
\label{tab:ablation_combined_new_metrics}
\end{table}

==> tables/ablations/tracking_vos.tex <==
\begin{table}[h]
\centering
% \resizebox will force the table to fit the column width.
% Note: This table is now wider, so \resizebox will shrink it more.
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l
                S[table-format=2.1]
                S[table-format=2.1]
                S[table-format=2.1]
                S[table-format=2.1]
                S[table-format=2.1]
                S[table-format=2.1]
                S[table-format=2.1]
                S[table-format=2.1]
                S[table-format=2.1]}
\toprule
% Abbreviated headers
\multirow{2}{*}{\textbf{Method}} & \multicolumn{3}{c}{\textbf{DAVIS}} & \multicolumn{3}{c}{\textbf{DAVIS (1080p)}} & \multicolumn{3}{c}{\textbf{SAV}} \\
% Add partial rules under the dataset names
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}
% Abbreviated sub-headers
& {J\&F} & {J} & {F} & {J\&F} & {J} & {F} & {J\&F} & {J} & {F} \\
\midrule
% --- Baselines ---
\multicolumn{10}{l}{\textit{Baselines}} \\
SAM2~\cite{sam2}        & \textbf{90.2} & {--} & {--} & 89.7 & 87.0 & 92.4 & \textbf{76.8} & {--} & {--} \\
Matanyone~\cite{matanyone}& 79.7          & 76.5 & 82.9 & 83.7 & 81.8 & 85.6  & 49.4          & 46.4 & 52.3 \\
\midrule
% --- Your Method + Ablations (New Order) ---
\multicolumn{10}{l}{\textit{Our Method (Ablations)}} \\
(a) ED & 77.0 & 74.1          & 80.0          & 78.5 & 75.6 & 81.4 & 45.9 & 42.5          & 49.4          \\
(b) Only Manual & 87.9 & 85.2 & 90.6          & 87.7 & 85.2 & 90.2 & 61.7 & 58.1 & 65.2          \\
(c) Manual+ED & 85.9 & 83.5 & 88.3 & 85.7 & 83.5 & 88.0 & 65.7 & 62.1 & 69.3 \\
(d) Auto+Manual+ED & 87.0 & \textbf{84.7} & \textbf{89.3} & 86.0 & 83.9 & 88.2 & 68.8 & \textbf{65.4} & \textbf{72.3} \\
\bottomrule
\end{tabular}%
} % End of \resizebox
\caption{
    Quantitative ablation on DAVIS val~\cite{davis}, DAVIS (1080p) val \& SAV val~\cite{sam2}.
    We report J\&F ($\mathcal{J}\&\mathcal{F}$), J ($\mathcal{J}$), 
    and F ($\mathcal{F}$). Best in \textbf{bold}.
    Our ablations: (a) w/o MAV, (b) Only Manual, (c) Auto+Manual (Full).
    ED denotes that existing dataset.
}
\label{tab:ablation_combined_final}
\end{table}
